A Host-SSD Collaborative Write Accelerator for LSM-Tree-Based Key-Value Stores

Log-Structured Merge (LSM) tree-based Key-Value Stores (KVSs) are widely adopted for their high performance in write-intensive environments, but they often face performance degradation due to write stalls during compaction. Prior solutions, such as regulating I/O traffic or using multiple compaction threads, can cause unexpected drops in throughput or increase host CPU usage, while hardware-based approaches using FPGA, GPU, and DPU aimed at reducing compaction duration introduce additional hardware costs. In this study, we propose KVACCEL, a novel hardware-software co-design framework that eliminates write stalls by leveraging a dual-interface SSD. KVACCEL allocates logical NAND flash space to support both block and key-value interfaces, using the key-value interface as a temporary write buffer during write stalls. This strategy significantly reduces write stalls, optimizes resource usage, and ensures consistency between the host and device by implementing an in-device LSM-based write buffer with an iterator-based range scan mechanism. Our extensive evaluation shows that for write-intensive workloads, KVACCEL outperforms ADOC by up to 1.17x in terms of throughput and performance-to-CPU-utilization efficiency. For mixed read-write workloads, both demonstrate comparable performance.

==> related.tex <==
\section{Related Work}

\subsection{Write-stall Mitigation for Key-Value Store}


\subsection{Key-Value SSD and Its Integration with Key-Value Store}
Since the introduction of the KV-SSD concept, numerous designs have emerged. 
KAML~\cite{jin2017kaml}, Samsung KVSSD~\cite{samsungKVSSD}, and iLSM-SSD~\cite{lee2019ilsm} have explored how to efficiently map key-value pairs to NAND pages within the device. 
PinK~\cite{im2020pink}, IterKVSSD~\cite{lee2023iterator}, and KV-CSD~\cite{kvcsd} have optimized the internal index data structures of KV-SSDs to further enhance key-value store functionality. 
However, none of these approaches attempted to integrate with existing host-side key-value stores like RocksDB.
Recently, Dotori~\cite{Dotori} and KVRangeDB~\cite{kvrangedb} have conducted studies on integrating host key-value stores with KV-SSDs. 
Dotori replaced the basic PUT/GET operations of the host key-value store with those of the KV-SSD, while KVRangeDB utilized the host-side LSM-tree iterator to improve range queries on KV-SSDs. 
However, neither of these studies addressed the use of KV-SSD from the perspective of write stall issues.
\kcache{} is the first to integrate KV-SSD with RocksDB, effectively resolving write stall problems and enhancing the utilization of both the device and the interconnect.

